APRIL: Active Preference-learning based Reinforcement Learning

This paper focuses on reinforcement learning (RL) with limited prior knowledge. In the domain of swarm robotics for instance, the expert can hardly design a reward function or demonstrate the target behavior, forbidding the use of both standard RL and inverse reinforcement learning. Although with a limited expertise, the human expert is still often able to emit preferences and rank the agent demonstrations. Earlier work has presented an iterative preference-based RL framework: expert preferences are exploited to learn an approximate policy return, thus enabling the agent to achieve direct policy search. Iteratively, the agent selects a new candidate policy and demonstrates it; the expert ranks the new demonstration comparatively to the previous best one; the expert's ranking feedback enables the agent to refine the approximate policy return, and the process is iterated. In this paper, preference-based reinforcement learning is combined with active ranking in order to decrease the number of ranking queries to the expert needed to yield a satisfactory policy. Experiments on the mountain car and the cancer treatment testbeds witness that a couple of dozen rankings enable to learn a competent policy.

==> Abstract.tex <==
Direct Policy Search with Ranking-based Approaches

\begin{abstract}
This paper handles direct policy search as an optimization problem, using
a monotonous estimate of the policy value as surrogate optimization objective.

This estimate can be extracted using learning-to-rank approaches, through exploiting 
the expert's (scarce) feedback. Ranking-based reinforcement learning applies beyond
the usual reinforcement learning settings: 
when reward functions can hardly be defined, such as in-situ robotics; or when
inverse reinforcement learning does not apply, as in swarm robotics. 

Furthermore, when dealing with a noisy policy value such as in the robotic keepaway problem, 
the use of monotonous estimates of the policy value leads to more robust policies. 

Experiments on the mountain car and the keepaway soccer testbeds show the merits and 
weaknesses of the rank-based policy learning approach.
\end{abstract}


==> abstractAPRIL.tex <==
\begin{abstract}
Motivated by in-situ robotics, this work tackles reinforcement learning with as light-as-possible
interaction with experts. Specifically, the considered setting involves no built-in reward 
function. The interaction with the expert is framed as a Learning-to-rank problem in
the policy space; iteratively, the robot demonstrates a policy, which is ranked by the expert 
comparatively to the previous policies. 

The contribution of the presented approach is to combine Active ranking with Reinforcement learning:
the robot learns an estimate of the expert's preferences, and demonstrates the most informative 
policy in the sense of this estimate.

The challenge is to reconcile two search spaces: the parametric policy space, and the behavioral
policy space. While the preference estimate can be learned from the behavioral space, the 
active learning criteria inspired from (Vappiani and Boutilier, 2010) are naturally defined on the 
parametric space. 

Experiments on standard benchmarks show the merits and the weaknesses of the {\em Active Preference-based 
Reinforcement Learning} scheme
compared to Inverse Reinforcement Learning.
\end{abstract}


==> algoAPRIL.tex <==
\section{APRIL Overview}
\label{sec:april}
\def\AA{\mbox{$\Pi$}}
\def\CC{$\cal C$}
\def\bev{{\em behavioral representation}}
\def\SM{SMS$(\pi)$} 
\def\PPL{{PPL}}

\def\At{{\mbox{$\cal A$$_t$}}}
\def\Jt{{\mbox{$J$$_t$}}}
\def\Jtp{{\mbox{$J^+$$_t$}}}
\def\Jtm{{\mbox{$J^-$$_t$}}}
\def\Ct{{\mbox{$C$$_t$}}}
\def\pit{{\mbox{$\pi^*$$_t$}}}
\def\pre{{rank-based policy estimate}}
\def\esp{\hspace*{.2in}}
\def\pix{\mbox{$\pi_x$}}

The Active Preference-based Reinforcement Learning algorithm iterates the following steps:\\
$\bullet$ Demonstrate a policy to the expert, and record whether it improves on the 
former best policy \pit. The policy archive is maintained, together with the ranking constraints;\\
$\bullet$  Determine the next candidate policy by optimizing criterion \Ct\ presented in section \ref{sec:C}, and iterate.\\

\subsection{Input and Feature spaces}

After \cite{PPL11}, APRIL considers two search spaces. The first 
one noted $X$, referred to as input space or parametric space, is suitable to generate and execute 
the policies. In the following $X = \RR^d$; policy \pix\ is represented by e.g. the weight vector $x$ 
of a neural net, mapping the current sensor values onto the effector values. 

The second space noted $\Phi(X)$, referred to as feature space or behavioral space, is suitable to 
learn the \pre. Taking inspiration from \cite{ORegan01}, the behavioral space is designed by discretizing 
the (sensor, motor) value vectors visited along the robot trajectory. To each sensori-motor cluster
is associated a feature, the value of which is set to the percentage of time spent in this cluster.
$\Phi(X) = [0,1]^D$, with $||\Phi(x)||_1 =1$. 
In contrast with the standard RL setting, the behavioral space does not reflect any prior knowledge
on the domain, or on the value function under estimation.

Archive \At\ is initialized with a random policies $\pi_0$ to be demonstrated to the expert. \At\ stores the input and the feature representation of the policies
(respectively noted $\pi_i$ and $\phi(\pi_i)$), together with the ranking constraints ($\pi_i \prec \pi_j$; without loss of generality, archive policies are ordered by increasing preference).

\subsection{Learning a rank-based policy estimate}\label{sec:J}

Using a standard constrained convex optimization formulation \cite{struct,Joachims_Implementation}, the \pre\ \Jt\ is sought as a linear mapping on $\Phi(X)$
\[ \Jt(\phi(\pi)) = \langle w_t,\phi(\pi) \rangle\mbox{~with~}w_t \in \Phi(X) \mbox{~ solution of $(P)$}\]

\[ (P) \left\{ \begin{array}{ll}
\mbox{Minimize } &\frac{1}{2}~||\mathbf{w}||^2 + C \sum_{i,j=1, i > j}^{t} \xi_{i,j}\\
\mbox{subject to } & 
(\langle\mathbf{w},\phi(\pi_{i})\rangle - \langle\mathbf{w},\phi(\pi_{j})\rangle \geq 1 - \xi_{i,j}) \\
& \mbox{ and } (\xi_{i,j} \geq 0), \mbox{ for all } 0 \le i < j \le |\At| 
\end{array}\right.\]

By construction, \Jt\ is independent on the policy parametric representation space, which might be relevant for transfer learning among different controller spaces (e.g. considering neural nets or central
pattern generators). Secondly and more importantly, \Jt\ provides some information 
about the relevance of a feature, akin the interpretation of 
a feature weight as a relevance score at the root of SVM-RFE \cite{Guyon-SVM-RFE}. 

A feature weight however differs from the standard RL value functions, in the sense that it 
does not reflect the expected cumulative reward related to the feature. In particular, it might increase
or decrease along the iterations, depending on whether this feature is discriminant for the policy quality comparatively to the policies considered so far.

\subsection{Active preference criterion}\label{sec:C}
The goal is to define a criterion enforcing the efficient exploration vs exploitation of the policy
space, suitable to select a candidate policy such that it maximizes the ultimate decision 
quality. The ideal criterion thus corresponds to the expected value of information \cite{Viappiani10}
(section \ref{sec:soa}).

As already mentioned however, the use of the Expected Improvement criteria \cite{EGO,Brochu}, or 
policy gradient methods are forcluded as \Jt\ is defined on the feature space $\Phi(X)$.
The input-to-feature space mapping only depends on the robot environment as a simulator-free setting is assumed, and solving the inverse feature-to-input space mapping is of the same order of 
difficulty as the RL problem {\em per se}. 

It thus comes to approximate the expected value of information of a policy $\pi$ as the sum of i) the value of the candidate solution, would it dominate the current best solution \pit; ii) the value of the current best solution \pit, would it dominate $\pi$. 

Denoting  \Jtp\ (respectively \Jtm) the \pre\ learned from \At\ augmented with the constraint
$\pi > \pit$ (resp. $\pi < \pit$), criterion \Ct\ is defined as:
\begin{equation}
  \Ct(\pi) = \Jtp(\pi) + \Jtm(\pit), \pi \not = \pit 
\label{eq:ct}
\end{equation}
This criterion intuitively corresponds to  the splitting index used in active learning \cite{Dasgupta05},
where the constraint $\pi<\pit$ splits the version space of the hypotheses satisfying all ordering constraints in the archive into two subsets. \Ct\ thus increases when none of these subsets is negligible, that is, when testing whether $\pi<\pit$ significantly decreases the version space.
In criterion $C_t$, the center of mass of the version space used in the Bayesian setting 
is approximated by the solution of the support vector machine problem (see \cite{HerbrichGC01} for an
extended comparison of the SVM and the Bayesian approaches).

In the meanwhile, it is clear that ordering constraints $\pi > \pit$ and $\pit > \pi$ are not equally probable given the current knowledge characterized by the set of constraints in $\At$. It is desirable to take their probabilities into account, along the same lines as the use of the belief state $\theta$ in section \ref{sub:bayes}. The simplest option would be to ignore $\Jtp$ or $\Jtm$ if any of them result in a solution that cannot satisfy all the constraints. However, this option may be too restrictive as it precludes the presence of any kind of noise, due to either the expert's preferences or the robot environment. Finally, terms $\Jtp$ and $\Jtm$ are weighted with the inverse of their objective value minimized in $(P)$, that is the sum of the associated $w$ and ranking error $\xi_{i,j}$. The higher this value, the worse the associated solution, and the lesser its weight is in criterion $C_t$.



==> algo_SML.tex <==
\section{APRIL Overview}
\label{sec:april}
\def\AA{\mbox{$\Pi$}}
\def\CC{$\cal C$}
\def\bev{{\em behavioral representation}}
\def\SM{SMS$(\pi)$} 
\def\PPL{{PPL}}

\def\At{{\mbox{$\cal A$$_t$}}}
\def\Jt{{\mbox{$J$$_t$}}}
\def\Jtp{{\mbox{$J^+$$_t$}}}
\def\Jtm{{\mbox{$J^-$$_t$}}}
\def\Ct{{\mbox{$C$$_t$}}}
\def\pit{{\mbox{$\pi^*$$_t$}}}
\def\pre{{rank-based policy estimate}}
\def\esp{\hspace*{.2in}}
\def\pix{\mbox{$\pi_x$}}
\def\zx{\mbox{{\bf z}$_x$}}
\def\phix{\mbox{$\phi(\pi_x)$}}

\def\w{\mbox{\bf w}}
\def\wp{\mbox{{\bf w}$^+$}}
\def\wn{\mbox{{\bf w}$^-$}}
\def\z{\mbox{\bf z}}
\def\zt{\mbox{{\bf z}$_t$}}
\def\zo{\mbox{{\bf z}$_0$}}
\def\zst{\mbox{{\bf z}$_t^*$}}


The Active Preference-based Reinforcement Learning algorithm (APRIL) is a two-step iterative 
process, alternating a demonstration and a self-training phases. In the demonstration phase, the selected policy is demonstrated to the expert, who ranks it comparatively to the current best policy \pit. The APRIL archive \At, including all demonstrated policies and ranking 
constraints, is updated accordingly. In the self-training phase, the agent determines the next candidate policy to be demonstrated to the expert. This candidate policy is the one maximizing criterion \Ct\ (section \ref{sec:C}).

\subsection{Input and Feature spaces}

After \cite{PPL11}, APRIL considers two search spaces. The first one noted $X$, referred to as input space or parametric space, is suitable to generate and run the policies. In the following $X = \RR^d$; policy \pix\ is represented by e.g. the weight vector $x$ of a neural net or the parameters of a control pattern generator (CPG) \cite{CPG}, mapping the current sensor values onto the actuator values. 

As mentioned, the parametric space however is hardly suitable to learn a preference-based 
policy return estimate, for the  agent behavior depends in an arbitrarily non-smooth
way on the parametric representation of its policy (due to the environment effects), 
while the expert's preferences only depend on the agent behavior. 
Another space, noted $\Phi(X)$ and referred to as feature space or behavioral space, thus is
considered in order to learn a \pre. The feature space considered in IRL \cite{Abbeel04} clearly relies on extensive prior knowledge. More generally, significant efforts have been made in RL to design a feature space suitable to capture the state-reward dependency (see e.g. \cite{HachiyaS10}). In the considered swarm robotics framework however, comprehensive prior knowledge is not available; and intensive simulated experiments are not affordable.
 
The alternative approach, inspired from \cite{ORegan01}, takes advantage of the fact that the agent is given for free the datastream made of its sensor and actuator values, generated along its
trajectories in the environment. A frugal online clustering algorithm approach (e.g. $\varepsilon$-means
\cite{Duda}) is used to define sensori-motor clusters. To each such cluster, referred to as sensori-motor
state (sms), is associated a feature. 
It thus comes naturally to describe a trajectory by the
fraction of overall time it spends in every sensori-motor state\footnote{The use of the time fraction is 
chosen for simplicity; one might use instead the {\em discounted} cumulative time spent in every sms.}.
Letting $D$ denote the number of sms, each trajectory \zx\ generated from \pix\ thus is represented as a unit vector in $[0,1]^D$ ($||\zx||_1 = 1$). The behavioral representation associated to \pix, noted \phix, finally is the distribution over $[0,1]^D$ of all trajectories \zx\ (reflecting the actuator and sensor noise, and the presence and actions of other robots in the swarm).

The main properties of the proposed behavioral representation is that it does not reflect any prior 
knowledge on the domain, nrqor on the value function to be learned\footnote{Further work is concerned with adaptively refining the clustering granularity, e.g. along the same lines as \cite{Oudeyer}.}. Moreover, it consistently accommodates the fact that the agent gradually discovers its sensori-motor space (e.g. considering new policies) by adding new sms features, the value of which is consistently set to 0 for earlier policies.  



\subsection{Learning a \pre}\label{sec:J}
The APRIL algorithm is initialized considering a random policy $\pi_0$ and a trajectory \zo\
demonstrating $\pi_0$. At time step $t+1$, a trajectory
of the candidate policy (selected in section \ref{sec:C}) is demonstrated to the expert, who indicates
whether this trajectory improves on the previous best trajectory \zst. 
At time $t$, archive \At\ stores the previous policies $\pi_i$ and the associated trajectories $\z_i$ demonstrated to the expert, for $i=0, \ldots t$, and the ranking constraints ($\z_i \prec \z_j$). Without 
loss of generality, the archive is ordered by increasing preference.

Using a standard constrained convex optimization formulation \cite{struct,Joachims_Implementation}, the \pre\ \Jt\ is sought as:
\[ \Jt(\pix) = \EE_{\z \sim \phix} [ \langle \w_t, \z \rangle]\mbox{~with~} \w_t \in [0,1]^D \mbox{~ solution of $(P)$}\]

%XX: la preference va croissant: i < i+1
\[ (P) \left\{ \begin{array}{ll}
\mbox{Minimize } F(\w) = &\frac{1}{2}~||\w||^2 + C \sum_{i,j=1, i > j}^{t} \xi_{i,j}\\
\mbox{subject to } & 
\langle\w,\z_j\rangle - \langle\w,\z_i)\rangle \geq 1 - \xi_{i,j} \\
& \mbox{ and } \xi_{i,j} \geq 0, \mbox{ for all } 0 \le i < j \le |\At| 
\end{array}\right.\]

By construction, \Jt\ is independent on the policy parametric representation space, which enables transfer learning among different controller spaces (e.g. transfer from neural nets to central pattern generators). Secondly and more importantly, \Jt\ provides some hints into 
the relevance of a sensori-motor state, akin the absolute value of a feature weight in linear SVM
can be used for feature selection \cite{Guyon-SVM-RFE}.
Likewise, if the $i$-th sms is associated a strongly positive (respectively negative) weight $w_i$, 
this sms can be interpreted as very beneficial (resp. detrimental) to the RL goal.
Note however that such weights cannot be interpreted in terms of the Q-value associated to some (state action) pair in mainstream RL: while $Q(s,a)$ is bound to increase along the value iteration steps, 
$w_i$ might increase or decrease along APRIL iterations, depending on whether the associated sms is visited by the best trajectories demonstrated so far. Typically, an excellent sms will be associated  a small weight if it is visited by all trajectories.


\subsection{Active preference criterion}\label{sec:C}
The goal is to define a criterion enforcing the efficient exploration vs exploitation of the policy
space, suitable to select a candidate policy such that it maximizes the ultimate decision 
quality. The ideal criterion thus corresponds to the expected value of information \cite{Viappiani10}
(section \ref{sec:soa}).
As already mentioned however, the use of the Expected Improvement criteria \cite{EGO,Brochu}, or 
policy gradient methods are forcluded as \Jt\ is not defined on the input parametric space. 
The input-to-feature space mapping only depends on the robot environment as a simulator-free setting is assumed, and solving the inverse feature-to-input space mapping is of the same order of 
difficulty as the RL problem {\em per se}. 

Let us consider a candidate policy \pix, and a trajectory \zx\ sampled after distribution \phix. This trajectory will be compared to the current best trajectory \zst, splitting the version space of all weight vectors consistent with the ranking constraints in the archive \At. (While we cannot assume a realizable setting, i.e. the expert's preferences are likely to be noisy \cite{Viappiani10}, the number of ranking constraints is always small relatively to the number $D$ of sensori-motor states. One can therefore assume that the version space defined from \At\ is not empty). This version space is thus divided into a so-called challenger version space noted $W^+$ (hypotheses ranking \zx\ higher than \zst), and its complementary $W^-$ (ranking \zst\ higher than \zx).

The expected utility selection of a candidate policy \pix\ is thus decomposed into the expectation over
all trajectories \zx\ of its expected \pre\ (where the expectation is taken over all $\w$ in the challenger version space $W^+$), and the \pre\ of the previous best trajectory \zst\ averaged on  
$W^-$:
\begin{equation} 
\begin{array}{ll}
EUS(\pix) = \EE_{\zx \sim \phix} \biggl[ \EE_{\w~in~W^+} [\langle \w,\zx\rangle] + \EE_{\w~in~W^-} [\langle \w,\zst\rangle] \biggr] \\
  \end{array}
\label{eq:eus}
\end{equation}


Taking the expectation over all weight vectors \w\ in $W^+$ or $W^-$ is clearly intractable as \w\ ranges in a high-dimensional continuous space. Two approximations are therefore 
considered. The first one consists of approximating the center of mass of a version space (that is,
the solution of the Bayes machine \cite{HerbrichGC01}) by the center of the 
largest ball in this version space (that is, the solution of the support vector machine). As 
extensively discussed in \cite{HerbrichGC01}, the SVM solution provides a good approximation of 
the Bayes machine solution provided the dimensionality of the space is ``not too high`` (more on this in section \ref{sec:artif}). The center of mass of 
$W^+$ (respectively $W^-$) is replaced by \wp\ (resp. \wn) the solution of the problem $(P)$ where \At\ is augmented with ranking constraint $\zx > \zst$ (resp. $\zx < \zst$). 
 
The second approximation takes care of the fact that constraint $\zx < \zst$ likely
divides the version space defined from \At\ into two subspaces $W^+$ and $W^-$ with different probabilities (said otherwise, the splitting index might be arbitrarily low). The expectation of $\langle\w,\zx\rangle$ thus requires 
the probability of $W^+$ and $W^-$ to be approximated. Along the same line as above, we use the inverse of the objective value $F(\wp)$ (respectively $F(\wn)$) to estimate the probability of $W^+$ (resp. $W^-$): the higher the objective value, the smaller the margin and the probability of the associated version space.

Finally, the approximate expected utility selection of a policy \pix\ is defined as:

\begin{equation}
  \Ct(\pix) = \EE_{\zx \sim \phix} \biggl[ \frac{1}{F(\wp)} \langle \wp,\zx\rangle + \frac{1}{F(\wn)} \langle \wn,\z\rangle] \biggr] 
\label{eq:ct}
\end{equation}


==> expe_SML.tex <==
\section{Goal of Experiments}
\label{sec:goal}
The first goal of the experiments is to assess the approximation of the expected utility selection 
described by criterion $C_t$. 

A key issue of the APRIL approach is to simultaneously consider a parametric or input space, and 
a behavioral or feature space. On the one hand, a high-dimensional continuous representation is 
required for the sake of expressivity, to yield performant policies; 
in the meanwhile, such an expressive input space makes it difficult to learn a \pre. This dilemma
is sidestepped in APRIL by simultaneously considering an input and a feature space, where the feature
space is meant to describe the policy behavior with a controllable accuracy, conducive to learning a sufficiently accurate \pre.

The price to pay for dealing with both search spaces lies in the two approximations needed to transform 
the expected utility of selection (Eq. \ref{eq:eus}) proposed by \cite{Viappiani10}  into a tractable criterion (Eq. \ref{eq:ct}), 
replacing the two centers of mass i.e. the solutions of the Bayes machines with the solutions of the 
support vector machines \cite{HerbrichGC01}, and estimating the splitting index from the objective values 
of the underlying SVM problems.
An artificial active learning problem will thus be considered in section \ref{sec:aeus} in order to 
empirically assess the goodness of this approximation.

The second goal of the experiments is to assess the performance of the APRIL approach
comparatively to that of inverse reinforcement learning (IRL, section \ref{sec:soa}) \cite{Abbeel04}. Both IRL and APRIL aim at learning the reward function and the sought policy through an iterative 
two-step processes. The main difference is that IRL is provided with an expert trajectory, whereas 
APRIL is provided with the expert feedback about the agent trajectories. The question thus becomes 
the ``expert sample complexity'', i.e. the number of expert feedbacks required by APRIL 
to yield a policy as good as the one provided by IRL. This question is answered by considering two RL benchmark problems (section \ref{sec:eAPRIL}), the well-known mountain car problem and the cancer treatment problem considered in \cite{Furnkranz11}. Note that 
none of these problems is associated with a reward function. 

\section{Empirical validation of criterion $C_t$}\label{sec:aeus}\label{sec:artif}
\begin{figure*}[t!]
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.5\textwidth]{figures/simplex_10.pdf}
&
\includegraphics[width=0.5\textwidth]{figures/simplex_20.pdf}\\
$d=10$ & $d=20$\\
\includegraphics[width=0.5\textwidth]{figures/simplex_50.pdf}
&
\includegraphics[width=0.5\textwidth]{figures/simplex_100.pdf}\\
$d=50$ & $d=100$\\
\end{tabular}
\end{center}
\caption{Performance of criterion $C_t$ vs expected utility of selection criterion 
comparatively to the random and Max-coordinate baselines (see text) versus the number of 
pairwise comparisons (number of expert feedbacks in APRIL), depending on dimension $d$. All results are averaged over 101 runs.}

\label{fig_simplex}
\end{figure*}
The experimental setting used to assess criterion $C_t$ is inspired from \cite{Dasgupta05}. A target ranking 
vector \w$^*$ is selected in the $d$-dimensional ball of radius 1 (considering norm $L_1$ instead of 
norm $L_2$ in \cite{Dasgupta05}). In each step ($x$ coordinate in Fig. \ref{fig_simplex}), the active
ranking candidate \w$_t$ is selected out of a fixed set $S$ of 1,000 points uniformly sampled in the $d$-dimensional unit ball; the quality of \w$_t$ is estimated from its scalar product with \w$^*$; lastly, the oracle provides a single bit of information, stating whether \w$_t$ improves on the current best solution. 
The criteria used to select the active ranking candidate \w$_t$ out of $S$ are as follows. 
The first one is criterion $C_t$ (Eq. \ref{eq:ct}). The second one is the approximated greedy EUS as defined by 
\cite{Viappiani12}. Formally, for each point $\w$ in $S$, 10,000 points $s$ are uniformly drawn in the 
version spaces $W^+$ and $W^-$, and the expectation $\EE_{\w~in~W^+}[\langle \w, s\rangle]$ is 
empirically estimated. Two baseline approaches are also considered. The random baseline uniformly selects 
\w\ in $S$ in each time step. The second baseline referred to as Max-Coord simply selects with no replacement \w\ with maximal infinite norm. 

Fig. \ref{fig_simplex} reports the performance of all four approaches averaged on 101 runs. It shows 
that the $C_t$ criterion used in APRIL yields a good approximation of the EUS, which gracefully degrades
as dimension $d$ increases: as noted in \cite{HerbrichGC01}, the approximation of the center of mass 
of the version space given by the center of the larger ball in the vs is less good as $d$ increases. 
%In the meanwhile, the computational cost of $C_t$ is lesser by XX orders of magnitude than that of EUS. 

Note that the approximate greedy EUS also degrades as dimension $d$ increases, due to the fact that a 
fixed size $S$ is considered. Unexpectedly, the Max-Coord baseline performs well in the early stages
of the active ranking process, all the more so as $d$ is small. It is thereafter dominated by all
other approaches (except the random baseline for low-dimensional spaces). The comparison with the 
Max-Coord baseline was meant to show that APRIL does not simply explore the extreme points in the 
simplex. 


\section{Empirical validation of APRIL}\label{sec:eAPRIL}\label{sec:resu}
This section reports on the empirical results of APRIL on the mountain car benchmark and the cancer
treatment problem. 

\subsection{Experimental setting}
APRIL is assessed comparatively to inverse reinforcement learning (section \ref{sec:soa}), legend Projection\_AL and 
to the stochastic optimization of $J_t(\pix)$ used in \cite{PPL11}, legend 1+11-ES (where the APRIL self-training phase is replaced by taking the 
best trajectory out of 11 trajectories, generated from policies obtained by Gaussian perturbations 
${\cal N}(0,\sigma)$ of the parametric representation of the policy that generated the best trajectory \zst\ found insofar). In the latter case, parameter $\sigma$ is initialized to $1$ and 
adjusted with a multiplicative increase (respectively decrease) factor $c=1.5$ (resp. $c^{1/4}$) when the deonstrated trajectory does (resp. does not) improve on the current best one.

Policies are implemented as 1-hidden layer neural nets, with 3 input nodes, 10 nodes on the hidden layer for the mountain car and 100 nodes on the hidden layer for the cancer treatment problem, and 1 output node (the acceleration for the mountain car and the dosage for the cancer treatment problem). The learning to rank algorithm is RankSVM \cite{Joachims_Implementation}, 
with linear kernel and $C = 100$.
All results are averaged out of 101 independent runs. 

\subsection{The cancer treatment problem}


In the cancer treatment problem, given an initial state of a patient, defined by its tumor size and toxicity, the goal is to adjust the medicine dosage for reducing tumor size without reaching a too high toxicity level.
The experimental setting is the same as the one used in \cite{Furnkranz11}, including the stochastic death mechanism, with
two differences. Firstly, the dosage level is a real value in $[0,1]$, as opposed to 4 discrete values in \cite{Furnkranz11}; secondly the time horizon is set to 12 (instead of 6 in \cite{Furnkranz11}). 
The initial state is set to 1.3 tumor size and 0 toxicity. 

% \begin{figure}[b!]
% \centerline{\includegraphics[width=0.45\textwidth]{figures/cancer.pdf}}
% \caption{Comparative performances of APRIL, IRL and stochastic optimization on the cancer treatment problem, plotting the cumulative toxicity level and tumor size after 12-months treatment, versus the number of trajectories demonstrated policies to the expert. Results are averaged over 101 runs}
% \label{fig_cancer}
% \end{center}
% \end{figure}

For the sake of reproducibility the expert preferences are emulated by favoring the trajectory with minimal sum of the tumor size and toxicity level at the end of the 12-months treatment. 
The results (averaged out of 101 runs, Fig.\ref{fig_cancer}) show how easy the problem is for inverse
reinforcement learning, which finds the optimal policy in the second iteration.  
A tentative interpretation for this fact is that the target behavior extensively visits the 
state with zero toxicity and tumor size; the learned \w\ thus associates a maximal weight to this 
state; in subsequent iterations, $\w$ thus favors policies reaching this state as soon as possible. 
APRIL catches up after 15 iterations, while the stochastic optimization remains consistently far 
from reaching the target policy in the considered number of iterations.

Additionally, we considered varying noise conditions in the cancer treatment problem by adding a Gaussian noise to the transition model defined in \cite{Furnkranz11} with the standard deviation $\sigma_{noise}$ being one of the values in \{0.05, 0.1, 0.2\}. To cope with the noise, the expected utility of selection is averaged over a fixed number of Monte-carlo runs (eleven runs resulting in eleven feature vectors for which the expected utility of selection is computed) for a given policy to get its associated $C_t$.  
A perspective for further research is to use racing methods, e.g. Bernstein races,  to estimate the confidence interval of the $C_t$ criterion in order to minimize the number of required Monte-carlo runs needed to determine with high probably the policy with the highest $C_t$, taking inspiration from  \cite{Verena09}.  

\begin{figure*}[t!]
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.5\textwidth]{figures/cancer.pdf}
&
\includegraphics[width=0.5\textwidth]{figures/cancer_noise005.pdf}\\
$\sigma_{noise}=0$ & $\sigma_{noise}=0.05$\\
\includegraphics[width=0.5\textwidth]{figures/cancer_noise01.pdf}
&
\includegraphics[width=0.5\textwidth]{figures/cancer_noise02.pdf}\\
$\sigma_{noise}=0.1$ & $\sigma_{noise}=0.2$\\
\end{tabular}
\end{center}
\caption{Comparative performances of APRIL, IRL and stochastic optimization on the cancer treatment problem, plotting the cumulative toxicity level and tumor size after 12-months treatment, versus the number of trajectories demonstrated to the expert, for various levels of noise. Results are averaged over 101 runs.}
\label{fig_cancer}
\end{figure*}

\subsection{The mountain car}

With same setting as in \cite{StoneRLEVO}, the car state is described from its position and speed, 
initially set to position  $-0.5$ with speed $0$. Its action is the car acceleration, varying in 
$\{-1, 0, 1\}$. For the sake of reproducibility the expert preferences are emulated by favoring the trajectory which soonest reaches the top of the mountain, or is closest to the top of the mountain at the time horizon of 1,000 time steps. 
Interestingly, the mountain car problem appears to be more difficult for IRL than
the cancer treatment problem (Fig.\ref{fig_mc}), which is explained from the lack of expert features.
As the trajectory is stopped when reaching the top of the mountain and this state does not appear in the trajectory histogram, the target reward would have negative weights on every (other) sms feature. 
IRL thus finds an optimal policy after 7 iterations on average. 
As for the cancer treatment problem, APRIL catches up after 15 iterations, while the stochastic 
optimization never catches up in the considered number of iterations. 

\begin{figure}
\centerline{\includegraphics[width=0.55\textwidth]{figures/mountain_car.pdf}}
\caption{Comparative performances of APRIL, IRL and stochastic optimization on the mountain car problem, plotting the number of time steps needed to reach the top of the mountain, versus the number of trajectories demonstrated policies to the expert. Results averaged over 101 runs}
\label{fig_mc}
\end{figure}


\section{Conclusion}
The main contribution of the presented paper compared to our previous work devoted to Preference-based 
Policy Learning \cite{PPL11} is to take inspiration and adapt recent advances in preference elicitation \cite{Viappiani12} in order to restrict the number of interactions with the expert needed to 
yield a good policy.

The lesson learned is that a very limited external information is required to enable reinforcement 
learning: while standard RL requires a numerical reward to be associated to each possible state in the 
search space, while inverse reinforcement learning requires the expert to demonstrate a sufficiently good 
policy, APRIL might require as few as one or two dozen bits of information (this trajectory improves/does not improve on the former best one) to reach state of the art results. 

Perspectives for further research are twofold. On the theoretical side, some theoretical analysis of the 
convergence of the approach and the approximation quality of the proposed criterion will be proposed. On the applicative side, APRIL will be experimented on large-scale problems such as the Robocup task where designing good reward functions raises significant difficulties. 

Another perspective is to consider multiple-instance ranking \cite{MIP}, to account for the fact
that the expert's preferences might be explained from {\em fragments} of the trajectory, 
as opposed to, from its overall histogram. 

% J'enleve celui-ci qui est trop copliqué
Yet another possibility is to consider hybrid policies, using the parametric policy description (e.g. NN weight vector) by default and exploiting the current estimate of the expert preferences on the top of it. Typically the estimate of the expert's preferences could be used to bypass the parametric policy, when e.g. it indicates that some action should be preferred to the parametric one in a given (discretized) state. 




==> experimentsAPRIL.tex <==
\section{Experimental Validation}
\label{sec:resu}
This section presents the experimental validation of APRIL.
\subsection{Goal of Experiments}
The goal of the experiments is to 
answer two questions. The first one regards the impact of criterion $C_t$, 
where the Bayesian formulation (considering the center of mass of the version space) is replaced by a 
SVM formulation \cite{HerbrichGC01}. 

The second one regards the performance of the APRIL approach
compared to Inverse Reinforcement Learning (IRL) \cite{Abbeel04}. Akin APRIL, IRL produces a sequence of policies, expectedly approximating the ideal one. The difference is that the information provided to IRL is significantly higher, since IRL is provided with a demonstration of the expert policy. 

The first question is investigated considering an artificial setting inspired from \cite{Dasgupta05}. 
On this setting, the greedy optimization of the \textit{expected utility of selection} ($EUS$) as proposed in \cite{Viappiani10} is compared to the APRIL criterion (Eq. \ref{eq:ct}), where the 
center of mass of the version space is approximated by Monte-Carlo sampling and averaging. 

The second question is answered by comparing APRIL to the \textit{projection algorithm}, an IRL  algorithm proposed in \cite{Abbeel04} on two reinforcement learning tasks, the well-known 
mountain car benchmark and the cancer treatment problem considered in \cite{Furnkranz11}. Note that 
none of these problems is associated with a reward function. 

\begin{figure*}[t!]
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.4\textwidth]{figures/simplex_10.pdf}
&
\includegraphics[width=0.4\textwidth]{figures/simplex_20.pdf}\\
\includegraphics[width=0.4\textwidth]{figures/simplex_50.pdf}
&
\includegraphics[width=0.4\textwidth]{figures/simplex_100.pdf}\\
\end{tabular}
\end{center}
\caption{Performances of criterion $C_t$ vs the approximate Bayesian approach (greedy-EUS), 
comparatively to two baselines (random and Max-Coordinate; see text), versus the number of 
pairwise comparisons (number of expert input in APRIL), in dimension $d=10$ (top left), $d = 20$ (top right), $d = 50$ (bottom left) and $n = 100$. All results are averaged over 101 runs.}
\label{fig_simplex}
\end{figure*}

\subsection{Synthetic data}
In this experiment a candidate set $S$ made of 1000 points uniformly sampled in the unit \textit{d-simplex} is considered. The difference w.r.t. \cite{Dasgupta05} is that we consider the sphere w.r.t. 
norm $L_1$ (points correspond to normalized histograms) whereas norm $L_2$ was considered in \cite{Dasgupta05}. The target solution $w^*$ is uniformly selected in the unit \textit{d-sphere} (with $d$ ranging in 10, 20, 50 and 100). The goal thus is to find its best approximation in $S$ ($argmax_{x \in S} <w^*, x>$). Note that the only ground truth provided is by means of pairwise comparisons between candidate points. The candidate point compared to the current best point $x^*_t$ in each time step is selected considering four approaches: 
\begin{enumerate}
\item APRIL selects in each iteration the point in $S$ which maximizes criterion $C_t$ (section \ref{sec:C}); this candidate point is compared with $x^*_t$, where the first point is randomly chosen.
\item Greedy-EUS \cite{Viappiani10} computes for each point $x$ in $S$ an approximation of the center of 
mass of the version spaces defined from respectively $x < x^*_t$ and $x > x^*_t$ (besides former pairwise comparisons). This approximation relies on a uniform sample of $10,000$ reward vectors $w$ consistent w.r.t. former pairwise comparisons.
\item Two simple baselines are also considered. The first one selects uniformly a candidate in $S$; the second one, referred to as Max-Coord selects the candidate point with maximal infinite norm. 
\end{enumerate}
From Fig.\ref{fig_simplex} we first note that the Max-Coord baseline that selects in priority points with a high value on a single coordinate performs well especially in the initial phase. As could have been expected, it is soon dominated by the other approaches as it does not take into account the former pairwise comparisons, all the more so as the dimension increases (note that it is dominated by
the random baseline for $d = 100$). The comparison shows that APRIL does not simply explore the extreme
points in the simplex.

After Fig. \ref{fig_simplex}, the $C_t$ criterion used in APRIL yields similar performances as 
the approximate Bayesian approach (Greedy-EUS), although at a considerably lesser computational cost. It is 
interesting to see that APRIL even dominates Greedy-EUS for $d = 20$ in the early stages, which is explained from the fact that the Monte-Carlo approximation of Greedy-EUS considers a 
fixed-size sample whereas dimension $d$ increases. In larger dimensions however ($d=50,100$), 
Greedy-EUS catches up. A tentative interpretation for this fact, based on \cite{HerbrichGC01}, 
is that the SVM approach finds the center of the largest ball in the version space: the approximation
of the true center of mass of the version space is less good as the dimension increases.


\subsection{Mountain Car and Cancer Treatment}
This section considers two RL problems: the mountain car benchmark and the cancer treatment problem. APRIL is compared with an apprenticeship learning algorithm (the projection algorithm \cite{Abbeel04}) that takes as input a demonstration of the optimal solution and then tries to uncover the policy that generated this behavior. The output of the algorithm is very similar to that of APRIL as it maintains an archive of policies (initially containing one random policy), where at each iteration, the reward maximizing the difference between the target behavior and the policies of the archive is selected, and the policy maximizing this reward is added to the archive. The process is iterated until we can assess that for any possible reward (and thus also the true reward), there is at least one policy in the archive that performs as well as the target behavior under this reward. Although we do not expect to do better than apprenticeship learning as we have no such input as a target behavior and we start by not having any information on the task, we at least hope that the number of required policies to demonstrate to the expert stay in the same order of magnitude as in the apprenticeship learning setting.

\begin{figure}[b!]
\includegraphics[width=0.45\textwidth]{figures/cancer.pdf}
\caption{Performance of the 3 compared methods on the cancer treatment problem, plotting the cumulation of the toxicity level and tumor size along the 12 months of treatment with a varying number of demonstrated policies to the expert. Results averaged over 101 runs}
\label{fig_cancer}
\end{figure}


In the cancer treatment problem, given an initial state of a patient, defined by its tumor size and toxicity, the goal is to adjust the medicine dosage for reducing tumor size without reaching a too high toxicity level. The experimental setting 
is the same as the one used in \cite{Furnkranz11} with the only differences of having a time horizon $H=12$ (the treatment duration is 12 months instead of 6), and the use of 
continuous actions (the dosage level is a real value in $[0,1]$, as opposed to 4 discrete values in \cite{Furnkranz11}). We set the initial state at 1.3 tumor size and 0 toxicity. While for mountain car we used the same settings found in \cite{StoneRLEVO}. We recall that this problem consists of controlling the acceleration of a car so that it can successfully climb a mountain. The state space consists of both the position and speed of the car while the action is the acceleration and can take one of the 3 values in $\{-1, 0, 1\}$. We set the initial state of the car at a position of $-0.5$ and a null speed.

In both problems, the policy is implemented as 1-hidden-layer feed-forward neural network with 3 inputs (a bias plus the current tumor size and toxicity for the cancer treatment problem or the position and speed for mountain car), 7 neurons in the hidden layer and 1 output being either the medicine dosage or the acceleration of the car. $C_t$, the criteria optimized by APRIL at each iteration makes use of $SVM^{rank}$  \cite{Joachims_Implementation} with linear kernel and $C = 100$.

During each optimization phase, eleven new policies are generated at each rounds, perturbing the 
current best policy $\pi_t$ using Gaussian noise ${\cal N}(0,\sigma)$, where $\sigma$ is initialized to $1$, with a multiplicative increase (respectively decrease) factor $c=1.5$ (resp. $c^{1/4}$) when the candidate policy does (resp. does not) improve on the former ones.

For the sake of reproducibility the expert preferences are emulated, favoring for the cancer treatment problem policies that reach the lowest sum of tumor size and toxicity level during the whole trajectory, and for mountain car the ones that reach the top the fastest or the one that get the closest to it after the 1000 time steps.  The presented results are averaged over 101 independent runs. APRIL performance is assessed comparatively to two baselines. The first one, referred to as {\em (1+11)-ES}, uses the same optimization algorithm as in APRIL (perturbing at each time the best policy so far with Gaussian noise) but with a criteria giving random values to the policies.
While the second one, {\em Projection-AL}, is the apprenticeship learning algorithm.

On the cancer treatment problem, Fig.\ref{fig_cancer} shows that the apprenticeship learning algorithm finds the optimal policy directly at the second demonstration (the first one being random). This is due to the fact that the target behavior spend most of his time in the state having zero toxicity and tumor size, and as the reward of the projection algorithm in its first iteration is simply the target histogram minus the histogram of the first random policy, the reward will have its highest coordinate the same as the one corresponding to this state which will make the optimization phase in the next iteration favor policies reaching this state as fast as possible which is in this case the optimal policy. The mountain car (Fig.\ref{fig_mc}) is in the contrary more difficult for the apprenticeship learning algorithm as when reaching the top of the mountain everything happens as if we were automatically transfered to an absorbing imaginary goal state with zero reward (and thus not appearing in the histogram) for the rest of the time steps. The hidden reward here would be one having negative value on all the coordinates and thus the optimal policy is the one closest to 0 (reaching the goal state as fast as possible). As for APRIL, albeit being slower than apprenticeship learning, it still manages to find for both problems good policies by demonstrating less than 15 behaviors to the expert. Compared to {\em (1+11)-ES}, APRIL performs significantly better in the cancer treatment problems, while it has a slower start on mountain car as it have the tendency to favor in the first iterations histograms with a high value on one of the coordinates while the optimal policy has an histogram very close to 0. However it catches up at around the 9th iteration and quickly surpass it.

\begin{figure}
\includegraphics[width=0.45\textwidth]{figures/mountain_car.pdf}
\caption{Performance of the 3 compared methods on the mountain car problem, plotting the average number of time steps needed to climb the mountain with a varying number of demonstrated policies to the expert. Results averaged over 101 runs}
\label{fig_mc}
\end{figure}

\section{Conclusion}
Taking inspiration from recent advances in preference elicitation, this paper proposed an algorithm aimed at solving reinforcement learning problems with minimal interaction with the expert; APRIL neither requires the hand definition of a reward function nor the availability of a demonstration by the expert of the optimal policy. Nonetheless, experimental evidence showed that within a small number of pairwise preferences over policies, we were able to recover near-optimal policies. 

Perspectives for further research are twofold. On the theoretical side, some theoretical analysis of the 
convergence of the approach will be achieved. On the applicative side, APRIL will be experimented on 
large-scale problems (e.g. the Robocup task) where designing good reward functions raises significant difficulties. 

 Yet another possibility is to consider hybrid policies, using the parametric policy description (e.g. NN weight vector) by default and exploiting the current estimate of the expert preferences on the top of it. Typically the estimate of the expert's preferences could be used to bypass the parametric policy, when e.g. it indicates that some action should be preferred to the parametric one in a given (discretized) state. 




==> introAPRIL.tex <==
\section{Introduction}
\label{sec:introduction}
Since the early 2000s, significant advances in reinforcement learning (RL) have been obtained 
through using direct expert's input (inverse reinforcement learning \cite{Ng-Russell2000}, learning by imitation \cite{Billard}, learning by demonstration \cite{Konidaris10}), assuming the expert's ability to
demonstrate quasi-optimal behaviors and to provide an informed representation. 

In 2011, new RL settings based on preference learning and allegedly less demanding for the expert
have been proposed, motivated by the  difficulty of calibrating the reward function \cite{Furnkranz11}, 
or the lack of authorized robotic simulators \cite{PPL11}. In \cite{Furnkranz11}, the expert's ranking input
is used to learn a rank-based value function, which is used to learn a policy akin an energy-based learning approach in the state $\times$ action space. In \cite{PPL11}, the expert's ranking input is used to learn a policy estimate; this estimate defines an optimization problem in the parametric policy 
space.

The present paper investigates the use of active preference learning \cite{Viappiani10} within 
preference-based reinforcement learning, more specifically addressing the latter optimization setting. 

The challenge is the following. According to \cite{PSR}, a complex policy $\pi$ can hardly be expressed in a ``naive`` state $\times$ action space for tractability reasons. The use of parametric policy representations,  e.g. considering the weight vector $w$ of a neural net ($w \in X = \RR^d$, with $d$ a few hundred),
has been thoroughly investigated in the literature (see e.g. \cite{PeterSchaal08}
among others). However, the mapping $\Phi$ from the parametric to the behavioral description of 
policies (from $w$ onto the actual {behavior} of the policy $\pi_w$)
is nothing like smooth. Small modifications of $w$ can entail arbitrarily large differences in $\pi_w$ 
behavior, depending on the robot environment (e.g. the tendency to turn right or left in front of an obstacle might have far fetched impact on the overall robot behavior). 
The parametric search space $X$ might thus be poorly suited to learning a policy 
estimate, as the expert's preferences are clearly related to the policy behavior, and the policy 
behavior is a complex mapping of its parametric representation\footnote{Policy gradient methods indeed face the same difficulties; their properties are conditioned by the smoothness of mapping $\Phi$ \cite{PeterSchaal08}.}. In other words, the policy estimate must be learned on some behavioral or feature space
$\Phi(X)$, to be defined. 

However, active preference criteria \cite{Viappiani10,Brochu} naturally refer to the learning 
search space. If they are thus defined on $\Phi(X)$, they are ineffective in order to directly 
explore the parametric representation $X$, unless the so-called inverse problem (from $\Phi(x)$ 
to $x$) be solved. The difficulty of this inverse mapping 
is known in the context of the famed kernel trick \cite{TsochantaridisJHA05}.
In the reinforcement learning setting, the control from the input (parametric) to the feature (behavioral) space is even more critical and less controlled, 
as  mapping $\Phi$ is mediated by the robot environment.

The contribution of this paper is to propose an approximate active preference-based criterion
complying with the input-to-feature space mapping, and to study its merits and weaknesses in the 
context of the proposed {\em Active Preference-based Reinforcement Learning} (APRIL) approach.
A proof of concept of APRIL is given on 2 benchmark problems.

This paper is organized as follows. Section \ref{sec:soa} discusses work related to 
preference-based reinforcement learning and active preference learning. Section \ref{sec:april}
gives an overview of APRIL. Section \ref{sec:goal} describes the experimental setting and reports
on the empirical validation of the approach. The paper concludes with a discussion and some perspectives
for further research.


==> intro_SML.tex <==
\section{Introduction}
\label{sec:introduction}
Since the early 2000s, significant advances in reinforcement learning (RL) have been obtained 
through using direct expert's input (inverse reinforcement learning \cite{Ng-Russell2000}, learning by imitation \cite{Billard}, learning by demonstration \cite{Konidaris10}), assuming the expert's ability to
demonstrate quasi-optimal behaviors and to provide an informed representation. 

In 2011, new RL settings based on preference learning and allegedly less demanding for the expert
have been proposed. In \cite{Furnkranz11}, the underlying motivation is the difficulty of calibrating
the reward function. A roll-out approach is used to learn a rank-based value function, which is used to learn a policy akin an energy-based learning approach in the state $\times$ action space. In \cite{PPL11}, the approach is motivated by reinforcement learning for swarm robotics, adversely 
affecting the use of simulator-based approaches. While the expert cannot demonstrate the target behavior, thus forcluding the use of inverse reinforcement learning, she can provide some feedback about the demonstrated policies; this feedback is used to learn a preference-based policy estimate. This estimate defines an optimization problem in the parametric policy space.

Resuming our earlier work \cite{PPL11}, the present paper investigates the use of active preference learning within preference-based reinforcement learning, taking inspiration from interactive optimization \cite{Brochu} and active ranking \cite{Viappiani10}. 

The difficulty is the following. Interactive optimization (respectively active ranking) proceed by learning a surrogate optimization objective (resp. a ranking hypothesis) on the search space. In the 
RL context, the natural search space is the state $\times$ action space.
According to \cite{PSR} however, complex policies can hardly be expressed in the ``naive`` state $\times$ action space for tractability reasons. The standard alternative is to use parametric policy representations,  e.g. considering the weight vector $x$ of a neural net ($x \in X = \RR^D$, with $D$ a few hundred), which have been thoroughly investigated in the literature (see e.g. \cite{PeterSchaal08}
among others). Such parametric representation space $X$ might however be poorly suited to learning a preference-based policy estimate. On the one hand,  the expert's preferences are more directly related to the policy behavior, than to its parametric representation.  On the other hand, the mapping $\Phi$ from the parametric to the behavioral description of policies (from $x$ onto the actual {behavior} of the policy $\pi_x$)
is nothing like smooth; small modifications of $x$ can entail arbitrarily large differences\footnote{Policy gradient methods indeed face the same difficulties; their properties are conditioned by the smoothness of mapping $\Phi$ \cite{PeterSchaal08}.} in $\pi_x$ 
behavior, depending on the robot environment (e.g. the tendency to turn right or left in front of an obstacle might have far fetched impact on the overall robot behavior). In other words, the preference-based policy estimate must be learned on some behavioral or feature space $\Phi(X)$, to be defined. 

Earlier interactive optimization \cite{Brochu} or active ranking \cite{Viappiani10} approaches therefore hardly apply: While the objective is learned on behavioral space $\Phi(X)$, one aims at iteratively finding the best candidate policy in parametric space $X$. The above approaches thus are ineffective, unless the so-called inverse problem (from $\Phi(x)$ 
to $x$) be solved. The difficulty of this inverse mapping 
is known in the context of the famed kernel trick \cite{TsochantaridisJHA05}.
In the reinforcement learning setting, the control from the input (parametric) to the feature (behavioral) space is even more critical and less controlled, 
as  mapping $\Phi$ is mediated by the robot environment.

The contribution of this paper is to propose an approximate active preference-based criterion
complying with the input-to-feature space mapping, and to study its merits and weaknesses in the 
context of the proposed {\em Active Preference-based Reinforcement Learning} (APRIL) approach.
A proof of concept of APRIL is given on two benchmark problems.

This paper is organized as follows. Section \ref{sec:soa} discusses work related to 
preference-based reinforcement learning and active preference learning. Section \ref{sec:april}
gives an overview of APRIL. Section \ref{sec:goal} describes the goals of the experimental validation. Section \ref{sec:resu} reports on the experimental setting and discusses the results. The paper concludes with some perspectives
for further research.


==> soaAPRIL.tex <==
\section{State of the art}
\label{sec:soa}
Assuming the reader's familiarity with the reinforcement learning setting 
\cite{Sutton_Barto_1998}, this section briefly reviews work related to preference-based reinforcement learning and to active preference learning. 

\subsection{Preference-based reinforcement learning}
Reinforcement learning classically considers a Markov decision process framework, described by its  state and action space respectively denoted $\cal S$ and $\cal A$, its transition model $p(s,a,s')$ stating 
the probability of arriving in state $s'$ after executing action $a$ in state $s$ ($p: {\cal S} \times {\cal A} \times {\cal S} \mapsto [0,1]$), and its reward function $r: {\cal S}\times{\cal A} \mapsto \RR$).

To our best knowledge, the use of preference learning in the field of reinforcement 
learning was only investigated in \cite{Furnkranz11} and \cite{PPL11}.
With motivations from the medical protocol application domain, \cite{Furnkranz11} is concerned with the difficulty of calibrating the reward function (what is the cost of the patient death?), 
in order to facilitate the RL process. The authors thus 
extend the classification-oriented approach first proposed by \cite{Lagoudakis} as follows. In a given state $s$, an action $a$ is assessed by executing the current policy until reaching a terminal state (rollout). On the basis of these assessments, actions can thus be ranked (conditionally to $s$, e.g. 
$a <_s a'$); these ranking constraints are exploited within a learning-to-rank algorithm
(e.g. RankSVM \cite{Joachims05}), yielding a ranking hypothesis $h_s$. The authors advocate that such action ranking hypotheses are more flexible than classification hypotheses, aimed at discriminating ``the'' best 
actions from the others conditionally to the current state. The main weakness of this approach seems
to be the necessity of learning a ranking hypothesis { per} state.

\cite{PPL11} is concerned by the robotic application domain, specifically focussing on swarm robotics. The authors argue that the swarm robotics context forbids the use of simulators due to the supra-linear
computational complexity of simulations w.r.t. the number of robots in the swarm.
%, and due to the simulation noise. 
It also forbids the 
inverse reinforcement learning approach \cite{Abbeel04,Kolter07}; in most cases the expert cannot describe (let alone demonstrate) the individual robot behavior leading to the desired swarm behavior (known as the inverse macro-micro problem \cite{Emergence}). They thus proceed along an interactive optimization setting: the robot(s) demonstrate
a behavior, which is ranked by the expert comparatively to the previous ones. The ranking constraints are likewise exploited within a learning-to-rank algorithm, yielding a ranking hypothesis $h$. The main difference is that $h$ refers to the overall policy behavior (macro-level), as opposed to the (state,action) space (micro-level). This hypothesis $h$ defines an optimization problem on the policy search space: find the optimal policy $\pi^*_h$ according to $h$. Policy  $\pi^*_h$ is demonstrated to the expert, who ranks it, and the process is iterated. The authors thus face the same difficulty as 
interactive optimization at large: if the expert is presented with a too constrained sample, she 
does not have a chance to teach her preferences to the system. 

\subsection{Active preference learning}
\label{sub:bayes}
This same problem of interactive optimization is faced by \cite{Brochu} and \cite{Viappiani10}, both
considering a Bayesian setting.

In \cite{Brochu}, the motivating application is to help the user quickly find a suitable visual rendering 
in an image synthesis context. The search space $X$ is made of the rendering parameter vectors.
The system displays a candidate solution, which is ranked by the user w.r.t. the previous ones. The ranking constraints are used to learn a Gaussian process (using a binomial probit regression model). 
The goal is to provide as quickly as 
possible a good solution, as opposed to, the optimal one. Accordingly, the authors use the Expected Improvement over the current best solution as optimization criterion, and they return the best vector out of a finite sample of the search space. They further note that returning the optimal solution, e.g. using the Expected Global Improvement criterion \cite{EGO} with a branch-and-bound method, raises 
technical issues on large search spaces.

In \cite{Viappiani10}, the context is that of recommendation systems. The system iteratively provides 
the user with a choice query, that is a (finite) set of solutions $S$, of which the user selects the
one she prefers. The ranking constraints are used to learn a utility function $w$, linear on the 
search space $X=\RR^D$. Within the Bayesian setting, the uncertainty about the utility function is expressed through a belief $\theta$ defining a distribution over the space of possible utility functions ($w \in \RR^D$).

Formally, the problem of (iterated) optimal choice queries is to simultaneously learn the user's utility function, and present the user with a set of good recommendations, such that she can select one with maximal expected utility. Viewed as a single-step (myopic) optimization problem, the goal thus boils down to finding a recommendation $x$ with maximal expected utility ($\EE_\theta[\langle w,x \rangle]$). 
In a sequential optimization perspective however \cite{Viappiani10}, the goal is to find a set of recommendations $S = \{x_1, \ldots, x_k\}$
with maximum expected {\em posterior utility}, defined as the expected gain in quality of the 
next decision. The expected utility of selection (EUS) is studied under several noise models, 
and the authors show that the greedy optimization of EUS provides good approximation guarantees of the 
optimal query. 

In \cite{Viappiani12}, the issue of the maximum expected value of information (EVOI) is tackled, and the authors consider the following criterion, where $x^*$ is the current best solution:
\[ \mbox{Select argmax} \{ \EE_{\theta, x > x^*}[\langle w,x \rangle] + \EE_{\theta, x <x^*}[\langle w,x^*\rangle ] \}   
\]
where the first term corresponds to the expected utility of $x$ conditionally to $x > x^*$, 
and the second term is the expected utility of $x^*$, conditionally to $x < x^*$.


==> soa_SML.tex <==
\section{State of the art}
\label{sec:soa}
Assuming the reader's familiarity with the reinforcement learning setting 
\cite{Sutton_Barto_1998}, this section briefly reviews work related to 
preference-based reinforcement learning and to active preference learning. We first briefly summarize inverse reinforcement learning for the sake of self-containedness.

\subsection{Inverse reinforcement learning}
Reinforcement learning classically considers a Markov decision process framework, described by its  state and action space respectively denoted $\cal S$ and $\cal A$, its transition model $p(s,a,s')$ stating 
the probability of arriving in state $s'$ after executing action $a$ in state $s$ ($p: {\cal S} \times {\cal A} \times {\cal S} \mapsto [0,1]$), and its reward function $r: {\cal S}\times{\cal A} \mapsto \RR$). A policy noted $\pi$ maps the state space onto the action space ($\pi: {\cal S} \mapsto {\cal A}$).

Inverse reinforcement learning (IRL) \cite{Abbeel04,Kolter07} considers a MDP without reward function, where the state space is mapped onto a vector of $k$ features $\phi$ ($\phi: {\cal S} \mapsto [0,1]^k$). 
Examples of such features are the instant speed of a driving policy or whether it bumps in a pedestrian.

Letting $s_0$ be the initial state, 
letting $\mu(\pi)$ denote the discounted expectation of the feature vector $\phi$ along policy $\pi$ (e.g. the discounted average speed), the target policy value is sought as a linear function of $\mu(\pi)$, i.e. it is defined by a weight vector $w$ such that:
\[ J(\pi) = \EE[V^\pi(s_0)] = \langle w, \mu(\pi) \rangle\] 
Interestingly, $w$ defines both the
policy return estimate {\em and} the reward attached to any state (since $r(s) = \langle w_t, \phi(s) \rangle$).

Let $\mu_E$ denote the empirical expectation of the feature vector $\phi$ along the expert demonstration.
IRL proceeds as a two-step iterative process, maintaining the set ${\cal A}_t$ of considered policies up to step $t$ (with ${\cal A}_0$ set to a random policy). In the first step,  the current weight vector $w_t$ is sought as the one maximizing the minimum of $\langle w, \mu_E - \mu(\pi_i) \rangle$, for $\pi$ ranging in ${\cal A}_t$. In the second step, policy $\pi_{t+1}$ is learned (by standard RL \cite{Abbeel04} or using Gibbs-sampling based exploration \cite{Kolter07}) from the current reward function defined by $w_t$. The process is iterated until reaching the desired approximation level.


\subsection{Preference-based reinforcement learning}

To our best knowledge, the use of preference learning in the field of reinforcement 
learning was only investigated in \cite{Furnkranz11} and \cite{PPL11}.
\cite{Furnkranz11} is concerned with the issue of calibrating the reward function in order to 
facilitate RL; for instance in the medical protocol application domains, how to associate a numerical negative reward to the patient's death ?  The authors thus 
extend the classification-oriented approach first proposed by \cite{Lagoudakis} as follows. In a given state $s$, an action $a$ is assessed by executing the current policy until reaching a terminal state (rollout). On the basis of these assessments, pairs of actions can be ranked conditioned by $s$ ($a <_s a'$); these ranking constraints are exploited within a learning-to-rank algorithm
(e.g. RankSVM \cite{Joachims05}), yielding a ranking hypothesis $h_s$. The claim is that such action ranking hypotheses are more flexible than classification hypotheses, aimed at discriminating ``the'' best 
actions from the others conditioned by the current state. The main weakness of this approach seems
to be the necessity of learning a ranking hypothesis { per} state.

\cite{PPL11} is concerned by the robotic application domain, specifically focussing on swarm robotics. The motivation is that the swarm robotics context forbids the use of simulators due to the supra-linear
computational complexity of simulations w.r.t. the number of robots in the swarm.
%, and due to the simulation noise. 
It also forbids the 
inverse reinforcement learning approach \cite{Abbeel04,Kolter07}; in most cases the expert cannot describe (let alone demonstrate) the individual robot behavior leading to the desired swarm behavior (known as the inverse macro-micro problem \cite{Emergence}). The proposed approach proceeds along an interactive optimization setting: the robot(s) demonstrate
a behavior, which is ranked by the expert comparatively to the previous ones. The ranking constraints are likewise exploited within a learning-to-rank algorithm, yielding a ranking hypothesis $h$. The main difference is that $h$ refers to the overall policy behavior (macro-level), as opposed to the (state, action) space (micro-level). This hypothesis $h$ defines an optimization problem on the policy search space: find the optimal policy $\pi^*_h$ according to $h$. Policy  $\pi^*_h$ is demonstrated to the expert, who ranks it, and the process is iterated. The authors thus face the same difficulty as 
interactive optimization at large: if the expert is presented with a too constrained sample, she 
does not have a chance to teach her preferences to the system. A heuristics is thus used to enforce the 
diversity of the policy sample demonstrated to the expert.

\subsection{Active preference learning}
\label{sub:bayes}
This same problem of interactive optimization is faced by \cite{Brochu} and \cite{Viappiani10}, both
considering a Bayesian setting.

In \cite{Brochu}, the motivating application is to help the user quickly find a suitable visual rendering 
in an image synthesis context. The search space $X$ is made of the rendering parameter vectors.
The system displays a candidate solution, which is ranked by the user w.r.t. the previous ones. The ranking constraints are used to learn a Gaussian process (using a binomial probit regression model). 
The goal is to provide as quickly as 
possible a good solution, as opposed to, the optimal one. Accordingly, the authors use the Expected Improvement over the current best solution as optimization criterion, and they return the best vector out of a finite sample of the search space. They further note that returning the optimal solution, e.g. using the Expected Global Improvement criterion \cite{EGO} with a branch-and-bound method, raises 
technical issues on large search spaces.

In \cite{Viappiani10}, the context is that of recommendation systems. The system iteratively provides 
the user with a choice query, that is a (finite) set of solutions $S$, of which the user selects the
one she prefers. The ranking constraints are used to learn a utility function $w$, linear on the 
search space $X=\RR^D$. Within the Bayesian setting, the uncertainty about the utility function is expressed through a belief $\theta$ defining a distribution over the space of possible utility functions ($w \in \RR^D$).

Formally, the problem of (iterated) optimal choice queries is to simultaneously learn the user's utility function, and present the user with a set of good recommendations, such that she can select one with maximal expected utility. Viewed as a single-step (myopic) optimization problem, the goal thus boils down to finding a recommendation $x$ with maximal expected utility ($\EE_\theta[\langle w,x \rangle]$). 
In a sequential optimization perspective however \cite{Viappiani10}, the goal is to find a set of recommendations $S = \{x_1, \ldots, x_k\}$
with maximum expected {\em posterior utility}, defined as the expected gain in quality of the 
next decision. The expected utility of selection (EUS) is studied under several noise models, 
and the authors show that the greedy optimization of EUS provides good approximation guarantees of the 
optimal query. 

In \cite{Viappiani12}, the issue of the maximum expected value of information (EVOI) is tackled, and the authors consider the following criterion, where $x^*$ is the current best solution:
\begin{equation}
  \mbox{Select argmax} \{ \EE_{\theta, x > x^*}[\langle w,x \rangle] + \EE_{\theta, x <x^*}[\langle w,x^*\rangle ] \} 
\label{eq:wvs}
\end{equation}

where the first term corresponds to the expected utility of $x$ conditioned by $x > x^*$, 
and the second term is the expected utility of $x^*$, conditioned by $x < x^*$.

This criterion can be analyzed by reference to active learning and the so-called splitting index criterion \cite{Dasgupta05}. Within the realizable setting (the target hypothesis $h^*$ belongs to the search space), the search only needs to explore the version space of all solutions consistent with the examples provided so far. Any instance $x$ splits the version space into two parts, respectively consistent with $h^*(x)=0$ and $h^*(x)=1$. The splitting index associated to $x$ is the minimum size of these two parts: the higher, the better. 

In active ranking, any instance $x$ likewise generates a constraint relatively to the current best instance $x^*$, which splits the version space into a challenger subset (the set of solutions ranking $x$ higher than $x^*$) and its complementary subset.
In optimal recommendation or interactive optimization, one must additionally consider the expectation
of the objective value of $x$ (more precisely, the expected fraction of instances which are ranked lower than $x$ by ranking hypotheses in the challenger subset); this expectation is captured by the first term in Eq. (\ref{eq:wvs}). 



